A Topology by Geometrization for Sub-Iterated Immediate Snapshot Message Adversaries and Applications to Set-Agreement

The Iterated Immediate Snapshot model (IIS) is a central model in the message adversary setting. We consider general message adversaries whose executions are arbitrary subsets of the executions of the IIS message adversary. We present a new topological approach for such general adversaries, based upon geometric simplicial complexes. We are able to define a topology directly on the considered sets of executions, which gives both simpler and more powerful ways of using topology for distributed computability. As application of this new framework, we present a complete characterization and lower bounds for solving set-agreement for general sub-IIS message adversaries.

==> sub-chr-2d.tex <==


\begin{tikzpicture}{thick}
  \useasboundingbox (0,0) rectangle (\textwidth,\lineheight));
  \node[proc,b] (bA) at (0,0) {};
  \node[proc,n] (nB) at (2,0) {};
  \node[proc,b] (bB) at (4,0) {};
  \node[proc,n] (nA) at (6,0) {};
  \draw (bA) -- (nB) -- (bB) -- (nA);
\end{tikzpicture}


==> sub-chr-3d.tex <==

\begin{tikzpicture}[thin]

  % triangle exterieur
  \draw (0.2, 0.737822173509) --
        (7.2, 0.737822173509) --
        (3.7, 6.8)            -- cycle;

  % bas
  \draw (0.2, 0.737822173509) -- (3.7, 1.95025773881);
  \draw (7.2, 0.737822173509) -- (3.7, 1.95025773881);
  \draw (4.86666666667, 0.737822173509) -- (3.7, 1.95025773881);
  \draw (2.53333333333, 0.737822173509) -- (3.7, 1.95025773881);

  % droite
  \draw (7.2, 0.737822173509) -- (4.4, 3.16269330411);
  \draw (3.7, 6.8) -- (4.4, 3.16269330411);
  \draw (4.86666666667, 4.77927405784) -- (4.4, 3.16269330411);
  \draw (6.03333333333, 2.75854811567) -- (4.4, 3.16269330411);

  % gauche
  \draw (3.7, 6.8) -- (3.0, 3.16269330411);
  \draw (0.2, 0.737822173509) -- (3.0, 3.16269330411);
  \draw (1.36666666667, 2.75854811567) -- (3.0, 3.16269330411);
  \draw (2.53333333333, 4.77927405784) -- (3.0, 3.16269330411);

  % triangle interieur
  \draw (4.4, 3.16269330411) node[proc,b]{} --
        (3.0, 3.16269330411) node[proc,n]{} --
        (3.7, 1.95025773881) node[proc,g]{} -- cycle;

  % noeuds
  \draw (0.2, 0.737822173509) node[proc,b]{};
  \draw (7.2, 0.737822173509) node[proc,n]{};
  \draw (3.7, 6.8)            node[proc,g]{};
  \draw (4.86666666667, 0.737822173509) node[proc,b]{};
  \draw (2.53333333333, 0.737822173509) node[proc,n]{};
  \draw (4.86666666667, 4.77927405784)  node[proc,n]{};
  \draw (6.03333333333, 2.75854811567)  node[proc,g]{};
  \draw (1.36666666667, 2.75854811567)  node[proc,g]{};
  \draw (2.53333333333, 4.77927405784)  node[proc,b]{};

\end{tikzpicture}

